Vizing's edge-recoloring conjecture holds

In 1964 Vizing proved that starting from any k-edge-coloring of a graph G one can reach, using only Kempe swaps, a ($\Delta$ + 1)-edge-coloring of G where $\Delta$ is the maximum degree of G. One year later he conjectured that one can also reach a $\Delta$-edge-coloring of G if there exists one. Bonamy et. al proved that the conjecture is true for the case of triangle-free graphs. In this paper we prove the conjecture for all graphs.

==> complexity.tex <==
\

==> cycles_around_v_starting_with_u.tex <==
\subsection[Cycles around \texorpdfstring{$v$}{v} starting with \texorpdfstring{$u$}{u}: a proof of Lemma~\ref{lem:cycles_around_v_starting_with_u}]{Cycles around \texorpdfstring{$v$}{v} starting with \texorpdfstring{$u$}{u}: a proof of\texorpdfstring{\break}{ }Lemma~\ref{lem:cycles_around_v_starting_with_u}}\label{sec:cycles_around_v_starting_with_u}



%{\Huge DEBUT}

In this section we prove Lemma~\ref{lem:cycles_around_v_starting_with_u}

\begin{proof}
The proof is done by induction on $i$. We handle the base case and the induction step respectively in Lemma~\ref{lem:base_case} and Lemma~\ref{lem:induction_step}. To prove the base case, we first prove the following claim.

\begin{claim}\label{cl:edge_between_u_u'}
Let $u = v_j$ and $u' = v_{j'}$ be two vertices of $\Vv$. If $\beta(uu')\neq c_v$, then $\Ww = X_v(\beta(uu'))$ is not a path.
\end{claim}

\begin{proof}

Otherwise, assume that $\Ww$ is a path. We can also assume that $\Ww$ is of length one, indeed if the length of $\Ww$ is more than one, we can invert it until we reach a coloring where it has length one without changing any color in $\Vv$ nor the color of $uu'$. We denote by $w'$ the only vertex of $\Ww$, and by $\beta'$ the coloring obtained after swapping the edge $vw'$. By Lemma~\ref{lem:fans_around_Vv}, $\Uu = X_u(c_{u'})$ and $\Uu' = X_{u'}(c_u)$ are cycles and $uu'$ is the last edge of each of these cycles; we denote by $w$ the vertex missing $\beta(uu')$ in $\Uu$. Clearly, $\beta(uu')\not\in\beta(\Vv)$, otherwise $\Ww = \Vv$ is a cycle and thus is not a path, as desired.
We first prove some basic properties on the fan $\Uu$.

\begin{proposition}\label{prop:no_edge_colored_with_c_in_beta(Vv)}
The fan $\Uu$ contains an edge colored $c_v$, and there is no edge colored with a color in $\beta(\Vv)$ between the edge colored $c_v$ and the edge colored $c_w$ in $\Uu$.
\end{proposition}
\begin{proof}
In the coloring $\beta'$, we have $m(v) = c_w$. If $\Uu$ does not contain any edge colored $c_v$, then $\Uu \neq X^{\beta}_u(c_v)$, and in the coloring $\beta'$, $X_u(c_{u'})$ contains a vertex $w'' \neq v$ missing the color $c_w = m(v)$, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in $\beta'$, and so it is in $\beta$. Therefore the only possible configuration is the following: the fan $\Uu$ contains the edge colroed $c_v$ incident with $u$, and does not contain any edge colored with a color in $\beta(\Vv)$ between this edge colored $c_v$ and the edge colored $c_w$, otherwise $\Uu$ is not entangled with $\Vv$ in $\beta'$ and by Lemma~\ref{lem:fans_around_Vv} $\Vv$ is invertible in $\beta'$, and so it is in $\beta$.
\end{proof}

\noindent Let $w_u$ be the neighbor of $u$ connected to $u$ by the edge colored $c_v$.

\begin{proposition}\label{prop:uw_u_and_u'w_u'_belong}
The edge $uw_u$ belongs to the component $K_v(c_v,c_{v_{j'-1}})$.
\end{proposition}
\begin{proof}
Assume that $uw_u$ does not belong to $K_v(c_v,c_{v_{j'-1}})$, and let\break $C = K_{uw_u}(c_v,c_{v_{j'-1}})$. If the vertex $w$ does not belong $C$, then we swap $C$ and obtain a coloring where $\Vv$ is still a minimal cycle but the fan $X_u(j'-1)$ is a now cycle that is not entangled with $\Vv$, so by Lemma\ref{lem:fans_around_Vv}, $\Vv$ is invertible in this coloring, and so it is in $\beta$. Therefore, the vertex $w$ belongs to the component $C$, and after swapping this component, we obtain a coloring where $\Vv$ is still a minimal cycle, and by Observation~\ref{obs:tight}, it is still tight. Thus, we can do a sequence swaps of the form $K_{w'}(t,t+1)$ for $t\in (j'-1,\cdots,j)$; these swaps may have changed the color of $uw_u$, but after the sequence of swaps, it is guaranteed that the color of $uw_u$ is in $\beta(\Vv)$. Note that, since $\Vv$ is tight, the last swap has not changed the colors of the edges incident with $u$. After this sequence of swaps, $m(w') = c_{u}$, and $\Vv$ is still saturated (otherwise, it is invertible in this coloring, and so it is in $\beta$), thus we swap $K_{w'}(c_v,c_u)$ without changing the color of any edge incident with $u$ or $v$, and it suffices to then swap the edge $vw'$ to obtain a coloring where $X_u(uw_u)$ is not a cycle entangled with $\Vv$, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in this coloring, and so it is in $\beta$; a contradiction.
\end{proof}

\begin{proposition}\label{prop:w'_in_k_w(c_u,c_w)}
In the coloring $\beta'$, the vertex $w'$ belongs to both $K_w(c_u,c_w)$ and $K_w(j-1,c_w)$, moreover, after swapping one of these components, $\Vv$ is still tight and saturated.
\end{proposition}
\begin{proof}
The proof of this proposition is straightforward, the two cases being similar, we only prove it for $K_w(c_u,c_w)$. Assume that $w'$ does not belong to\break $K_w(c_u,c_w)$, then we swap this component and swap the edge $vw'$ to obtain a coloring where $X_u(c_v)$ is not entangled with $\Vv$, a contradiction by Lemma~\ref{lem:fans_around_Vv}. So $w'$ belongs to this component, and after swapping it, the fan $\Vv$ is still a cycle of the same size, so it is tight and saturated by Observation~\ref{obs:tight} and Lemma~\ref{lem:saturated_cycles} respectively, otherwise, it is invertible in this coloring, and so it is in $\beta$.
\end{proof}

\noindent We can now conclude the proof of the claim, but we have to distinguish whether or not $u$ and $u'$ are consecutive in $\Vv$ ($\ie$ whether or not $j = j'+1$).
\setcounter{case}{0}
\begin{case}[$j = j'+1$]
~\newline
 In the coloring $\beta'$, we consider the component $C_w = K_w(c_w,c_u)$; this component contains the vertex $w'$ by Proposition~\ref{prop:w'_in_k_w(c_u,c_w)}. After swapping $C_w$ we obtain a coloring where the fan $X_u(c_v)$ is a path. Note that in this path, no edge between $uu_2$ and $uw$ can be colored with a color in $\beta(\Vv)$ by Proposition~\ref{prop:no_edge_colored_with_c_in_beta(Vv)}. So we invert this path, and no edge colored with a color in $\beta(\Vv)$ has been changed during the inversion. In the coloring obtained after the inversion, we have that the component $C_{u'} = K_{u'}(c_{u'},c_v)$ contains $w_u$ and does not contain $uw_u$ and $uv$ anymore. After swapping $C_{u'}$, we obtain a coloring where $m(u') = m(u) = c_v$, and we swap the edge $uu'$ to obtain a coloring where the fan $X_v(m(u))$ is a path that we invert. In the coloring obtained after the inversion, we have that the component $K_w(c_w,c_u)$ is exactly $C_w\cup\{uw\}$ so we swap it to obtain a coloring where $m(u) = m(v)$. Note that swapping back $C_w$ before $C_{u'}$ does not interfere with the previous swap of $C_{u'}$ as $|\{c_u,c_w,c_v,c_{u'}\}| = 4$. In the coloring obtained after the swap, we swap the edge $uv$ to obtain a coloring where $X_u(c_w)$ is a path that we invert. In the coloring obtained after the inversion, we have that the component $K_{u'}(c_{u'},c_v)$ is an even cycle, more precisely it is exactly $C_{u'}\cup\{uu'\}\setminus \{uu_2\}$, and we swap it to obtain a coloring where $K_v(c_z,\beta(uv)) = \{vu',uu'\}$; after swapping this component we obtain exactly $\Vv^{-1}(\beta)$.
\end{case}

\noindent We now handle the case where $j\neq j'+1$.

\begin{case}[$j \neq j'+1$]
~\newline
For this case, we need to distinguish the cases based on the shape of\break $C = K_{uw_u}(c_v,c_{v_{j'-1}})$. By Proposition~\ref{prop:uw_u_and_u'w_u'_belong}, $C$ also contains $v$ and $v_{j'-1}$ in $\beta$, and so this component is a path in this coloring. There are two cases, in the coloring $\beta$, either $C$ is such that $u$ is between $v_{j'-1}$ and $w_u$, or $w_u$ is between $v_{j'-1}$ and $u$. We start both cases by swapping $C_1 = K_w(c_w,c_u)$, by Proposition~\ref{prop:w'_in_k_w(c_u,c_w)} the vertex $w'$ belongs to this component, and after the swap we have $m(w) = m(w')= m(u) = c_u$, so by Proposition~\ref{prop:no_edge_colored_with_c_in_beta(Vv)} $X_u(c_v)$ is a path that we invert without changing any color of $\Vv$, nor the color of the edge $uu'$, we denote by $\beta''$ the coloring obtained after the inversion. In the coloring $\beta''$, depending on the shape of $C$, either $u$ is in $C_2 = K_{v_{j'-1}}(c_v,c_{v_{j'-1}})$, or $w_u$ belongs to this component, and we now have to distinguish the cases. Both cases are pretty similar, their proofs rely on the same principle: apply Kempe swaps to reach a coloring where the edges of $E(\Vv)\cup\{vw'\}$ induce two fans that are cycles smaller than $\Vv$ (and so that are invertible by the minimality of $\Vv$).

\begin{subcase}[$u$ belongs to $C_2$]
~\newline
In this case, from the coloring $\beta''$, we swap the component $C_2$ to obtain a coloring where the fan $X_v(c_{v_{j'-1}}) = (vv_{j'},vv_{j'+1},\cdots,vv_{j-1},vv_{j})$ is a cycle strictly smaller that $\Vv$, so by minimality of $\Vv$, this cycle is invertible. Moreover, the fan $X_v(c_u) = (vv_{j+1},\cdots,vv_{j'-1})$ is also a cycle strictly smaller than $\Vv$, and so it is also invertible. After inverting these two cycles, we obtain a coloring where the component $K_{v_{j'-1}}(c_v,c_{v_{j'-1}}) = C_2 \cup \{vv_{j'-1},vu\}$ is an even cycle that we swap back. Moreover, the component $C_3 = K_{w_u}(c_v,c_{v_{j'-1}})$ is now a path containing $u'$, and we also swap it. After the swaps of these two components, the fan $X_v(c_{u'}) = (vu',\cdots,vu)$ is now a cycle strictly smaller than $\Vv$, so we invert it. In the coloring obtained after this inversion, by Proposition~\ref{prop:w'_in_k_w(c_u,c_w)}, the component $C_4 = K_{v_{j-1}}(c_{v_{j-1}},c_u)$ is now a path containing $v_{j-1}$ and $v_{j+1}$ but not the vertex $v$, and thus we swap it to obtain a coloring where the fan $X_v(c_v) = (vu',\cdots, vv_{j-1},vw')$ is a cycle strictly smaller than $\Vv$, therefore we invert it. In the coloring obtained after the inversion, the component $K_{w_u}(c_v,c_{v_{j'-1}})$ is now exactly $C_3$, and we swap it back to obtain a coloring where $X_u(c_u)$ is now a path that we invert. After inverting this path, the component $K_{v_{j-1}}(c_{v_{j-1}},c_u)$ is now exactly $C_4 \cup\{vv_{j-1},vu\}$ and we swap it back to obtain a coloring where the component $K_w(c_w,c_u)$ is exactly $C_1$. Finally we swap back this component to obtain exactly $\Vv^{-1}(\beta')$, and it suffices to swap the edge $vw'$ to obtain $\Vv^{-1}(\beta)$.
\end{subcase}
\begin{figure}[h]
\centering
\includegraphics[scale=0.3]{figures/kempe_case_1.png}
\caption{Subcase 2.1: the Kempe chain are represented by the purple dotted lines.}
\end{figure}

\begin{subcase}[$w_u$ belongs to $C_2$]
~\newline
In this case, from the coloring $\beta''$, we swap the component $C_2$ to obtain a coloring where $X_v(c_u) = (vv_{j+1},\cdots,vw')$ is a cycle strictly smaller than $\Vv$, so it is invertible. After inverting it, by Proposition~\ref{prop:w'_in_k_w(c_u,c_w)} we obtain a coloring where the the component $C_3 = K_{v_{j-1}}(c_{v_{j-1}},c_u)$ is now a path containing $v_{j-1}$ and $v_{j+1}$ but not the vertex $v$, and thus we swap it to obtain a coloring where $X_v(c_v) = (vv_{j'-1},\cdots,vu)$ is a cycle stricly smaller than $\Vv$, so it is invertible. After inverting it, the component $C_4 = K_{u'}(c_v,c_{v_{j'-1}})$ is now a cycle containing $vu$ and $vu'$, and after swapping this component, we obtain a coloring where the fan $X_v(c_v) = (vu',\cdots,vw')$ is now a cycle strictly smaller than $\Vv$, and thus we invert it. After inverting it, we obtain a coloring where the component $K_{v_{j'-1}}(c_v,c_{v_{j'-1}})$ is exactly $C_2$, and thus we swap it to obtain a coloring where the fan $X_v(c_{v_{j'-1}}) = (vu,\cdots,vv_{j'-1})$ is now a cycle strictly smaller than $\Vv$, and so we invert it. After inverting it, we obtain a coloring where the component $K_{u'}(c_v,c_{v_{j'-1}})$ is now exactly $C_4\setminus\{vu,vu'\}$, and we swap it back to obtain a coloring where $X_u(c_v)$ is a path that we invert. After inverting it, we obtain a coloring where the component $K_{v_{j-1}}(c_{v_{j-1}},c_u)$ is $C_3\cup \{vv_{j-1},vu\}$ and we swap it back to obtain a coloring where the component $K_w(c_w,c_u)$ is exactly $C_1$. After swapping back this component, we obtain exactly $\Vv^{-1}(\beta')$, and it suffices to swap the edge $vw'$ to obtain $\Vv^{-1}(\beta)$.


\end{subcase}
\begin{figure}[h]
\centering
\includegraphics[scale=0.3]{figures/kempe_case_2.png}
\caption{Subcase 2.2.}
\end{figure}
\end{case}

\end{proof}
\noindent We now prove Lemma~\ref{lem:cycles_around_v_starting_with_u}, as mentioned above we handle the base case, and the induction step in two separate lemmas. Both proofs are organized as a series of claims and their structure are similar. It is essentially a case analysis based on which type of fan (path, comet or cycle) these two fans induce.

% we first prove that the fans $\Ww$ and $\Zz$ are not paths, then that they are not a comets, and finally that they contain the respective mentioned vertices.

\begin{lemma}[base case, $w = u_{l-2}$]\label{lem:base_case}
~
\begin{itemize}
    \item $\Ww$ is a saturated cycle containing $w$, and 
    \item $\Zz$ is a cycle entangled with $\Vv$ containing $z$.
\end{itemize}
\end{lemma}

\begin{proof}
We first prove that $\Ww$ is a saturated cycle. By Claim~\ref{cl:edge_between_u_u'}, $\Ww$ is not a path. We now prove that the fan $\Ww$ is not a comet.

\begin{claim}
The fan $\Ww$ is not a comet.
\end{claim}
\begin{proof}
Otherwise assume that $\Ww$ is a comet, and let us denote by $w'$ an $w''$ the vertices of $\Ww$ missing the same color $c$, moreover, we assume that $w'$ is before $w''$ in $\Ww$. Clearly if $c \in \beta(\Vv)$, as $\Vv$ is saturated, $K_v(c,c_v)$ contains $w''\in\Vv$ and does not contain $w'$, so it suffices to swap $K_{w'}(c,c_v)$ to reduce this case to case where $\Ww$ is a path. Note that even if $u\in K_{w'}(c,c_v)$, in the coloring obtained after swapping this component, $c_z$ is still the color of the last edge of $\Uu$.
So $c\not \in \beta(\Vv)$, and we have that the vertices $w'$ and $w''$ are not both part of $K_v(c,c_v)$. Without loss of generality, we can assume that $w'\not\in C_v = K_v(c,c_v)$. We can swap $C_v$ to obtain a coloring where $X_v(c_z)$ induces a path, this case is also handled by the previous case. Similarly to the last case, the fact that whether $u\in C_v$ or not does not change the reasoning.
\end{proof}


\noindent So the fan $\Ww$ is a cycle, we now prove that it is saturated.

\begin{claim}
The fan $\Ww$ is saturated.
\end{claim}
\begin{proof}

Otherwise, assume that there exists $w'\in \Ww$ missing a color $c$ with $w'\not\in K_v(c,c_v)$. If $c \neq c_w$, similarly to the case where $\Ww$ is a comet, we can swap $K_{w'}(c,c_v)$ to obtain a coloring where $X_v(c_w)$ is a path. So $c = c_w$, and we have that $u\in C_{w'} = K_{w'}(c_v,c_z)$, otherwise it suffices to swap this component to reduce this case to the case where $\Ww$ is a path. Moreover, we also have that $w\in C_{w'}$, otherwise, it suffices to swap $C_{w'}$, and to invert the path $X_v(c_z)$ in the coloring obtained after the swap to obtain a coloring where $X_u(c_{u'})$ is not entangled with $\Vv$ since $w \not \in \Vv$. Thus by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in this coloring and so it is in $\beta$. So we swap $C_v = K_v(c_v,c_w)$; this component is different from $C_{w'}$, and so does not contain $u$ nor $w$ nor $w'$. After swapping this component , we obtain a coloring where $X_u(c_{u'})$ is not entangled with $\Vv$ because $w\not\in\Vv$, hence $\Vv$ is invertible in this coloring by Lemma~\ref{lem:fans_around_Vv}, so it is also invertible in $\beta$.
\end{proof}

\noindent So the fan $\Ww$ is a saturated cycle, we now prove that $\Ww$ also contains the vertex $w$.


\begin{claim}
The fan $\Ww$ contains the vertex $w$.
\end{claim}
\begin{proof}
Otherwise, assume that there exists $w' \in \Ww$ with $m(w') = m(w)$ and $w'\neq w$. As $\Ww$ is saturated, we have that $C_w = K_{w}(c_w,c_v)\neq K_v(c_w,c_v) = C_v$, and $w'\in C_v$. Moreover, $u\in C_w$, otherwise, it would suffice to swap it to obtain a coloring, where $X_u(c_{u'})$ is not entangled with $\Vv$, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in this coloring, and so it is in $\beta$. So $u$ is not in $C_v$, and if we swap $C_v$, we obtain a coloring where $X_u(c_{u'})$ is not entangled with $\Vv$; a contradiction by Lemma~\ref{lem:fans_around_Vv}.
\end{proof}

\noindent This concludes the part of the proof concerning the fan $\Ww$, we now prove that $\Zz$ is a cycle entangled with $\Vv$ containing $z$. Similarly to the previous claims, we first prove that $\Zz$ is not a path.

\begin{claim}\label{cl:base_case_z_not_path}
The fan $\Zz$ is not a path.
\end{claim}
\begin{proof}
Otherwise, assume that $\Zz$ is a path. If $w\in\Vv$, then by Lemma~\ref{lem:fans_around_Vv} $\Vv$ is invertible as desired. So $w\not\in \Vv$. As $\Zz$ is a path then we can invert it until we reach a coloring where $m(w)\in\beta(\Uu)\cup\beta(\Vv)$ and obtain a coloring where $X_u(c_{u'})$ is either a comet or is not entangled with $\Vv$, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible.

\end{proof}

\noindent So $\Zz$ is not a path, to prove that $\Zz$ is not a comet, we first prove that $\Zz$ is entangled with $\Vv$.

\begin{claim}\label{cl:base_case_z_entangled}
The fan $\Zz$ is entangled with $\Vv$.
\end{claim}

\begin{proof}
Otherwise, assume that there exists $z'\in\Zz$ with $m(z')\in \beta(\Vv)$ and $z'\not\in\Vv$, we furthermore assume that $z'$ is the first such vertex in $\Zz$. We now need to distinguish the cases depending on the missing color of $z'$.
\setcounter{case}{0}
\begin{case}[$c_{z'} = c_v$]
~\newline
In this case, as $\Ww$ is saturated, we have that $z' \not \in K_v(c_v,c_w)$. Moreover, we have that $u\in K_{z'}(c_v,c_z)$, otherwise it suffices to swap this component to obtain a coloring where $X_w(m(u))$ is a path, which correspond to the case of the previous claim. So $u\not\in K_v(c_v,c_w)$, hence, if we swap this component, we obtain a coloring where $X_w(m(u))$ induces a path that we invert until we reach a coloring where $m(w)\in\beta(\Vv)$. In the coloring obtained after the inversion, $X_v(m(u)) = \Vv$ is still a minimal cycle, and $X_u(m(u'))$ is either a path or is not entangled with $\Vv$, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in this coloring, and so it is in $\beta$.


% so $u\in K_v(c_u,c_w)$, and so $w$ does not belong to this component. Hence we can swap this component to obtain a coloring where $X_v(c_v)$ is a path that we can invert to obtain a coloring where $X_v(\beta(uu'))$ is a path; by Claim~\ref{cl:edge_between_u_u'} this is a contradiction.
\end{case}
\begin{case}[$c_{z'} = c_u$]
~\newline
In this case as $\Vv$ is saturated, $z'\not\in K_v(c_v,c_u)$, so we can swap $K_{z'}(c_v,c_u)$ to obtain a coloring similar to the previous case where $m(z') = c_v$.

\end{case}

\begin{case}[$c_{z'} \not\in\{c_u,c_v\}$]
~\newline
In this case, there exists $x$ such that $c_{z'} = c_{v_x}$, and since $\Vv$ is tight, we apply a sequence of Kempe swap of the form $K_{z'}(h,h+1)$ with $h\in(x,\cdots,j-1)$ to obtain a coloring where $m(z') = c_u$, which corresponds to the previous case.
\end{case}

\noindent So $\Zz$ is entangled with $\Vv$, we now prove that $\Zz$ is not a comet.

\begin{claim}
The fan $\Zz$ is not a comet.
\end{claim}
\begin{proof}
Otherwise, there exists $z'$ and $z''$ in $\Zz$ missing the same color $c'$, we assume that $z'$ is before $z''$ in $\Zz$. Again, if $w\in \Vv$, then by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible, so $w\not\in \Vv$. Moreover, from the previous claim, we derive that $c'\not\in \beta(\Vv)$, otherwise $\Zz$ is not entangled with $\Vv$. The vertices $z'$ and $z''$ does not both belong to $K_v(c',c_v)$, without loss of generality, we can assume that $z'\not\in K_v(c',c_v)$, and so we can swap $K_{z'}(c',c_v))$ to obtain a coloring where $X_w(m(u))$ is not entangled with $\Vv$; a contradiction by the previous claim.
\end{proof}

\noindent So $\Zz$ is a cycle, and since $\Zz$ is entangled with $\Vv$, it contains the vertex $u$ and a vertex missing the color $c_z$, we now prove that $M(\Zz,c_z) = z$.

\begin{claim}
The fan $\Zz$ contains the vertex $z$.
\end{claim}
\begin{proof}

Otherwise, assume that there exists a vertex $z'$ in $\Zz$ different from $z$ with $m(z') = m(z) = c_z$. We first consider the components of $K(c_z,c_w)$. The vertex $z'$ belongs to $K_w(c_w,c_z)$; otherwise we swap $K_{z'}(c_w,c_z)$ and obtain a coloring where $X_w(m(u))$ is a path; a contradiction by Claim~\ref{cl:base_case_z_not_path}. So $z' \in K_w(c_w,c_z)$, and $z\not\in K_w(c_w,c_z)$. Now the vertex $w$ belongs to $K_{z}(c_w,c_z)$, otherwise, we swap $K_{z}(c_w,c_z)$ to obtain a coloring where $z$ is now the last but one vertex of $X_u(m(u'))$, but $z$ is not in $X_v(m(z))$. Therefore the vertex $v$ is in $K_{z}(c_w,c_z)$. After swapping this component, we have that $z$ is the last vertex of $X_u(m(u'))$, so it is contained in $X_v(m(z))$, and moreover, $m(z) = c_w$. This means that in the coloring $\beta$, $z$ belongs to the cycle $X_v(c_z)$.
We now consider the components of $K(c_v,c_z)$ in the coloring $\beta$. Again, the vertices $z$ and $z'$ are not both part of $K_v(c_v,c_z)$. If $z'$ is not in $K_v(c_v,c_z)$, then we swap $K_{z'}(c_v,c_z)$ to obtain a coloring where $X_w(m(u))$ is not entangled with $\Vv$, so by Claim~\ref{cl:base_case_z_entangled}, $\Vv$ is invertible (whether $u\in K_{z'}(c_v,c_z)$ or not). So $z'\in K_v(c_v,c_z)$, and $z\not\in K_v(c_v,c_z)$, moreover, $u\in K_{z}(c_v,c_z)$, otherwise, it suffices to swap this component to obtain a coloring where $X_u(m(u'))$ is a path, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in this coloring and so it is in $\beta$. So after swapping $K_{z}(c_v,c_z)$ we obtain a coloring where $X_v(c_z)$ is a path (since it was a cycle in $\beta$), and after inverting it, we obtain a coloring where $X_w(m(u))$ is not entangled with $\Vv$; a contradiction by Claim~\ref{cl:base_case_z_entangled}.
\end{proof}


\end{proof}

\noindent We now prove Lemma~\ref{lem:induction_step} which corresponds to the induction step.
\begin{lemma}[induction step]\label{lem:induction_step}
~
Let $i> 1$, if for any $k<i$:
\begin{itemize}
    \item $X_v(c_{u_{l-1-k}})$ is a saturated cycle containing $u_{l-1-k}$, and
    \item $X_{u_{l-1-k}}(c_u)$ is a cycle entangled with $\Vv$ containing $u_{l-2-k}$.
\end{itemize}
Then:
\begin{itemize}
    \item $\Ww = X_v(c_w)$ is a saturated cycle containing $w$, and
    \item $\Zz = X_w(c_u)$ is a cycle entangled with $\Vv$ containing $z$.
\end{itemize}
where $w = u_{l-1-i}$, and $z = u_{l-2-i}$ are two consecutive vertices of $\Uu$.
\end{lemma}

\begin{proof}


Similarly to the base case, we first prove that $\Ww$ is a cycle containing $w$ by proving that $\Ww$ is not a path.

\begin{claim}\label{cl:induction_step_w_not_path}
The fan $\Ww$ is not a path.
\end{claim}
\begin{proof}
Otherwise, assume that $\Ww$ is a path, as $\Vv$ is a cycle, we have $c_w\not\in\beta(\Vv)$. By the induction hypothesis, all the vertices of $\Uu$ after $w$ are neighbors of $v$, so we can assume that $\Ww$ is of length one, we denote by $w'$ the vertex of this path, and by $\beta'$ the coloring obtained after swapping the edge $vw'$. In the coloring $\beta'$, the fan $X_{u}(c_{u'})$ is not entangled with $\Vv$ as it contains $w \not\in\Vv$ with $m(w) = m(v) = c_w$, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in $\beta'$, and so it is in $\beta$.
\end{proof}

\noindent We now prove that $\Ww$ is not a comet.

\begin{claim}
The fan $\Ww$ is not a comet.
\end{claim}

\begin{proof}
Otherwise, assume that $\Ww$ is a comet, and let us denote by $w'$ and $w''$ the vertices of $\Ww$ missing the same color $c$, we also assume that $w'$ is before $w''$ in $\Ww$. We now need to distinguish the cases depending on $c$. We denote by $\beta(\Uu_{>w})$ the set of colors of the edges of $\Uu$ that are after the edge $uw$ in $\Uu$.

\setcounter{case}{0}
\begin{case}[$c\in \beta(\Vv)\cup\beta(\Uu_{>w})$]
~\newline
In this case, since $X_v(c)$ is a saturated cycle by the induction hypothesis, and $w''\in X_v(c)$, the vertex $w''$ belongs to $K_v(c,c_v)$. Hence $w'$ is not in $K_v(c_v,c)$, so we can swap $K_{w'}(c,c_v)$ to obtain a coloring where $X_v(c)$ is a path, and therefore $\Vv$ is invertible in this coloring, and so it is in $\beta$. Note that the fact that $u$ belongs to $K_v(c,c_v)$ does not change the reasoning.
\end{case}

\begin{case}[$c\not\in \beta(\Vv)\cup\beta(\Uu_{>w})$]
~\newline
In this case, the vertices $w'$ and $w''$ cannot be both part of $K_v(c,c_v)$. Without loss of generality, we can assume that $w'$ is not in $K_v(c,c_v)$. We swap $K_{w'}(c,c_v)$ to obtain a coloring where $X_v(c)$ is a path, so in this coloring, $\Vv$ is invertbile by the induction hypothesis, and so it is in $\beta$.

\end{case}
\end{proof}

\noindent So the fan $\Ww$ is a cycle, we now prove that it is saturated.
\begin{claim}\label{cl:induction_step_w_sat}
The fan $\Ww$ is saturated.
\end{claim}
\begin{proof}
Otherwise, assume that there exists a vertex in $\Ww$ missing the color $c$ such that this vertex does not belong to $K_v                                              (c,c_v)$, we denote by $w'$ this vertex, and by $w''$ the vertex just after $w$ in $\Uu$. As $\Vv$ is a cycle, $c\not\in\beta(\Vv)$. Since $\Ww$ is not saturated, we swap the component $C_{w'} = K_{w'}(c,c_v)$ to obtain a coloring $\beta'$ where $w''$ is still the $(i-1)^{th}$ to last vertex of $X_u(c_{u'})$. If $u\not \in C_{w'}$ or $c\not\in\beta(\Uu)$, then $X_u(m(u'))$ is unchanged in $\beta'$ (it is exactly the edges of $\Uu$), and the fan $X_v(c_w)$ is a path in this coloring. So $\Vv$ is invertible in $\beta'$ by the induction hypothesis and so it is in $\beta$. Hence the vertex $u$ is in $C_{w'}$ and $c\in\beta(\Uu)$, we now have to distinguish the cases depending on the color $c$; we denote by $z'$ the vertex missing the color $c$ in $\Uu$. If $z'$ is after $w$ in the fan $\Uu$, then by the induction hypothesis, $X_v(c)$ is a saturated cycle containing $z'$, a contradiction, so either $c_{z'} = c_w$ or $z'$ is before $w$ in $\Uu$. If $z'$ is before $w$ in $\Uu$, then after swapping $K_{z'}(c,c_v)$ we obtain a coloring where $w$ is still the $(i-1)^{th}$ vertex of $X_u(m(u'))$, but where $X_v(m(w))$ is a path, so $\Vv$ is invertible by Claim~\ref{cl:induction_step_w_not_path} $\Vv$ is invertible in this coloring, and so it is in $\beta$. Hence $c_{z'} = c_w$, and after swapping $K_{z'}(c_w,c_v)$ we obtain a coloring where $X_v(c_w)$ is a path; after inverting this path, we obtian a coloring where $\Vv$ is still a minimal cycle, and where $X_u(c_{u'})$ is not entangled with $\Vv$, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in this coloring, and so it is in $\beta$.

% If $z'$ is after $w$ in $\Uu$, then in the coloring $\beta'$, $X_u(m(u'))$ is not entangled with $\Vv$, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in $\beta'$, and so it is in $\beta$.



% If $c\neq c_w$, then, as $w''$ is still the $(i-1)^{th}$ vertex of $X_u(m(u'))$ in $\beta'$, and $X_v(c)$ is a path in $\beta'$, then $\Vv$ is invertible in $\beta'$ by the induction hypothesis, and so it is in $\beta$. Hence $c = c_w$, and as $u\in C_{w'}$, we directly have that $w''\in C_{w'}$. It suffices to invert $X_v(c_x)$ to obtain a coloring similar to the previous case with the role of $c_v$ and $c_w$ switched, hence $\Vv$ is invertible in this coloring, and so it is in $\beta$.
\end{proof}

\noindent So $\Ww$ is a saturated cycle, we now prove that it also contains the vertex $w$.

\begin{claim}
The fan $\Ww$ contains the vertex $w$.

\end{claim}

\begin{proof}
Otherwise assume that there exists a vertex $w'\in\Ww$ different from $w$ missing the color $c_w$. As $\Ww$ is a saturated cycle, we have that $v\in K_{w'}(c_w,c_v)$, and so $w\not\in K_{w'}(c_w,c_v)$. So we swap the component $C_w = K_w(c_w,c_v)$ to obtain a coloring $\beta'$ where $m(w) = c_v$. We also have that $u$ belongs to $C_w$ and $c\in\beta(\Uu)$, otherwise the fan $X_u(m(u'))$ is not entangled with $\Vv$ and so $\Vv$ is invertible in $\beta'$ by Lemma~\ref{lem:fans_around_Vv}, and so it is in $\beta$. So $u$ is in $C_w$ and $c_v\in\beta(\Uu)$, and hence $w''$ is also $C_w$. In the coloring $\beta'$, we have that $w''$ is still the $(i-1)^{th}$ to last vertex of $X_u(m(u'))$, so $X_v(m(w''))$ is a saturated cycle containing $w''$, otherwise $\Vv$ is invertible by the induction hypothesis. So $w'' \in K_{v}(c_v,m(w''))$, and hence $w$ is not in $K_v(c_v,m(w'')$, and neither is $u$. So we swap $K_w(c_v,m(w''))$ to obtain a coloring where $X_{w''}(m(u))$ is a path (since it is a cycle containing $w$ in the coloring $\beta$ by the induction hypothesis) that we invert until we reach a coloring where $m(w'')\in\beta(\Vv)$. In the coloring obtained after the inversion, $X_u(m(v))$ is not entangled with $\Vv$, so by Lemma~\ref{lem:fans_around_Vv}, $\Vv$ is invertible in this coloring, and so it is in $\beta$.



% to obtain a coloring where $w''$ is missing the color $c_w$, we denote by $\beta''$ this coloring. In the coloring $\beta''$, $w''$ is still the $(i-1)^{th}$ to last vertex of $X_u(m(u'))$, but $X_v(m(w''))$ does not contain $w''$, so $\Vv$ is invertible in $\beta''$, and so it is in $\beta$.
\end{proof}

\noindent This concludes the part of the proof regarding the fan $\Ww$.
\end{proof}


\noindent We now prove that $\Zz$ is a cycle entangled with $\Vv$ containing $z$, we first prove that $\Zz$ is not a path.

\begin{claim}\label{cl:induction_step_z_not_path}
The fan $\Zz$ is not a path.
\end{claim}

\begin{proof}
Otherwise, if $\Zz$ is a path, then we can invert it until we reach a coloring where $m(z)\in \beta(\Vv)\cup\beta(\Uu_{<z})$ (where $\beta(\Uu_{<z})$ denotes the set of colors of the edges of $\Uu$ that comes before $uz$ in $\Uu$); in this coloring, $X_u(m(u'))$ is either a comet or is not entangled with $\Vv$, so $\Vv$ is invertible in this coloring by Lemma~\ref{lem:fans_around_Vv}, and so it is in $\beta$.
\end{proof}

\noindent We now prove that $\Zz$ is entangled with $\Vv$.

\begin{claim}\label{cl:induction_step_z_entangled}
The fan $\Zz$ is entangled with $\Vv$.
\end{claim}
\begin{proof}
Otherwise, assume that there exists a vertex $w'$ in $\Zz$ not in $\Vv$ which misses a color $c$ in $\beta(\Vv)$. We now need to distinguish the cases depending on $c$.
\setcounter{case}{0}
\begin{case}[$c = c_v$]
~\newline
In this case, as the cycle $X_v(c_w)$ is saturated, we have that $w'\not\in K_v(c_w,c_v)$. We can swap the component $C_{w'} = K_{w'}(c_v,c_w)$ to obtain a coloring $\beta'$ where $X_{w}(m(u))$ is a path. In the coloring $\beta'$, the vertex $w$ is still the $(i-1)^{th}$ to last vertex of $X_u(m(u'))$, and since $X_{w}(m(u))$ is a path, $\Vv$ is invertible in $\beta'$ by the previous claim, and so it is in $\beta$.
\end{case}

\begin{case}[$c  = c_u$]
~\newline
In this case, since the fan $\Vv$ is saturated, we have that $w'$ does not belong\break to $K_v(c_v,c_u)$. Since nor $u$ nor $v$ belongs to $C_{w'}$, we can swap $C_{w'} = K_{w'}(c_v,c_u)$ to obtain a coloring similar to the previous case, so $\Vv$ is invertible in this coloring and so it is in $\beta$.
\end{case}

\begin{case}[$c  \not\in\{c_v,c_u\}$]
~\newline
In this case, there exists $x$ such that $m(w') = c_{v_x}$, and since the fan $\Vv$ is tight, we can apply a sequence of Kempe swaps of the form $K_{w'}(h,h+1)$ with $h\in(x,\cdots,j)$ to obtain a coloring where $m(w') = m(u)$ and where no edge incident with a vertex of $\Vv$ has changed. This coloring is similar to the previous case, so $\Vv$ is invertible in this coloring and so it is in $\beta$.
\end{case}


\end{proof}

\noindent We now prove that $\Zz$ is not a comet.

\begin{claim}
The fan $\Zz$ is not a comet.
\end{claim}
\begin{proof}
Otherwise, there exist two vertices $z'$ and $z''$ in $\Zz$ missing the same color $c$ with $z'$ being before $z''$ in $\Zz$. By the previous claim, the color $c$ is not in $\beta(\Vv)$. We now consider the component $K_v(c,c_v)$. The vertices $z'$ and $z''$ cannot be both part of $K_v(c_v,c_w)$. Without loss of generality, we can assume that $z'$ is not in $K_v(c_v,c)$, so we swap the component $C_{z'} = K_{z'}(c,c_v)$, and we denote by $\beta'$ the coloring obtained after the inversion. In the coloring $\beta'$, we have that $w$ is still the $(i-1)^{th}$ to last vertex of $X_u(m(u'))$, but $X_{w}(m(u))$ is not entangled with $\Vv$, so $\Vv$ is invertible in $\beta'$ by Claim~\ref{cl:induction_step_z_entangled}, and so it is in $\beta$.
\end{proof}


\noindent Therefore, the fan $\Zz$ is a cycle, we now prove that it contains $z$.

\begin{claim}
The fan $\Zz$ contains the vertex $z$.
\end{claim}
\begin{proof}
Otherwise, assume that there exists $z'\in\Zz$ different from $z$ with $m(z') = m(z)$. We first consider the component $K_w(c_w,c_z) = K_u(c_w,c_z)$. The vertices $z$ and $z'$ cannot be both part of this component. If $z'$ is not in $K_w(c_w,c_z)$, then we can swap $K_{z'}(c_w,c_z)$ to obtain a coloring where $X_w(m(u))$ is a path, however, $w$ is still the $(i-1)^{th}$ vertex of $X_u(m(u'))$ in this coloring, so $\Vv$ is invertible in this coloring by Claim~\ref{cl:induction_step_z_not_path}, and so it is in $\beta$.

Therefore, the vertex $z'$ belongs to $K_w(c_w,c_z)$, and so $z$ is not in this component. We clearly have that $v$ belongs to $C_z = K_z(c_w,c_z)$, otherwise, after swapping $C_z$, we obtain a coloring where $X_v(c_w)$ does not contain $z$ which is the $(i-1)^{th}$ to last vertex of $X_u(m(u'))$. We denote by $\beta'$ the coloring obtained after swapping $C_z$. In the coloring $\beta'$, we have that $X_v(c_w)$ is a saturated cycle containing $z$. Let $w''$ be the vertex just after $w$ in $\Uu$ in the coloring $\beta$. By the induction hypothesis, in the coloring $\beta$, the fan $X_{w''}(c_u)$ is a cycle containing $w$, so in in the coloring $\beta'$, it is still the case. By the induction hypothesis, $\Vv$ is invertible in $\beta'$, and so it is in $\beta$.




% , so $K_{z'}(c_w,c_v))$ does not contain $v$ nor $w$





% . Moreover, since in the coloring $\beta$, $X_v(c_w)$ is a cycle containing $w$, in the coloring $\beta'$, $X_v(c_z)$ is a cycle containing $w$. Hence we can swap $C_w = K_w(c_w,c_z))$ to obtain a coloring where $X_w(m(u))$ is a path that we can invert to obtain a coloring where $X_v(c_z)$ is a path. After inverting this path, we obtain a coloring where $X_{w}(m(u))$ is not entangled with $\Vv$ and $w$ is still the $(i-1)^{th}$ to last vertex of $X_u(m(u'))$, so $\Vv$ is invertible in this coloring, and so it is in $\beta$. Note that the fact that $u$ belongs to $C_w$ or not does not change the reasoning.
\end{proof}

\noindent Hence, the fan $\Zz$ is a cycle entangled with $\Vv$ containing $z$ as desired. This concludes the proof.


\end{proof}


\end{proof}




%{\Huge fin}

==> definition.tex <==
\section{Notation and technical setup}

We inherit the technical setup of \cite{triangle free case}.
The graph $G$ is $\chi'-regular$, $\alpha$ is the optimal target coloring, and $\beta$ is the starting $(\chi'+1)$-coloring, and the proof is an induction on $\chi'$ where we align successively the color classes of $\alpha$ and $\beta$.

\begin{itemize}
\item $[\Delta+1]= \{1\cdots,\Delta+1\}$
    \item $K^\beta(a,b)$ is the induced subgraph of $G$ induced by the colors $a$ and $b$.
    \item $K^\beta_x(a,b)$ with $x\in V(G)\cup E(G)$ is the component of $K(a,b)$ containing $x$.
    \item $m(v)$ with $v\in V(G)$ is the missing color at $v$. When there is no ambiguity, we will drop the superscript.
    \item $X_v(y)$ with $y$ in $[\Delta+1]$ (resp. in $E(G)$ or $V(G)$) is the fan around $v$ starting at the edge colored $y$ (resp. starting at the edge $y$ or $vy$).
    \item $M(X,c)$ with $X$ being a fan, and $c\in[\Delta+1]$ is the vertex of $X$ missing the color $c$ if it exists.
    \item If $X$ is a fan around $v$ which induces a cycle in a coloring $\beta$, then $X_\beta^{-1}$ is called the invert of $X$, and is a coloring where $\forall e \not \in X$, $\beta(e) = X_\beta^{-1}(e)$, and $\forall xv \in X$, $X_\beta^{-1}(vx) = m_{\beta}(x)$, and $m_{X^{-1}} = \beta(vx)$. When there is no ambiguity, we will drop the subscript.
    \item Inverting $X$ is applying a sequence of Kempe changes to transform $\beta$ into $X^{-1}$.
    \item If $X$ is a fan around $v$ that induces a path, and $x\in X$ is a neighbor of $v$, then partially inverting $X$ up to $x$ is applying the sequence of trivial Kempe changes on the edges of $X$ until we reach a coloring $\beta'$ where $m_{\beta'}(v) = m_{\beta}(x)$.
    Inverting $X$ is just partially inverting it up to the first vertex of $X$.
    \item Let $X$ be a fan around a vertex $v$, and $\beta$ a coloring: $\beta(X)$ denotes the set of colors of the edges of $X$, and $m(X)$ denotes the set of the colors missing at a vertex of $X$, \ie~ $m(X) = \beta(X)\cup\{m(v)\}$.
    
\end{itemize}
Let $c$ be the color, and let $M= \alpha^{-1}(c)$. Let $e$ be an edge:
\begin{itemize}
    \item If $e\in M$ and $\beta(e) =c$ then $e$ is called $\emph{good}$
    \item If $e\in M$ and $\beta(e)\neq c$, then $e$ is called $\emph{bad}$
    \item If $e\not \in M$ and $\beta(e) = c$, then $e$ is called $\emph{ugly}$.
\end{itemize}

A coloring is minimal if it minimizes the number of bad edges, and then the number of ugly edges. We consider $\beta$ to be a minimal coloring.

==> easy_observations.tex <==

\section{First observations}
From $\cite{bonamy2021vizing}$, we have that in the coloring $\beta$ we have a vertex $v$ incident with bad edge $vv_0$ s.t. $X_v(vv_0)$ is a cycle, and $vv_1$ is an ugly edge. We denote by $\Vv = (vv_0,\cdots, vv_{k-1})$ this fan. Our goal will be to invert \Vv so that we get a contradiction with the minimality of $\beta$.

\begin{definition}
Let $S\subseteq V(G)\cup E(G)$, a Kempe change is $S$-stable if it does not change the colors of the edges of $S$, nor the missing colors of the vertices of $S$. Two coloring $\beta$ and $\beta'$ ar $S$-equivalent if there exists a sequence of $S$-stable Kempe change to pass from $\beta$ to $\beta'$.
\end{definition}

\begin{observation}
Let $X$ be a cycle in a coloring $\beta$, and let $\beta'$ be a coloring $X$-equivalent to $\beta$, $X$ is invertible in $\beta$ if and only if $X$ is invertible in $\beta'$.
\end{observation}
The proof of this observation is straightforward.

\begin{definition}
A cycle $X$ around a vertex $v$ is called saturated if for any $u\in X$, $v\in K_u(m(u),m(v))$.
\end{definition}

From $\cite{bonamy2021vizing}$, we have that if a cycle $X$ around a vertex $v$ is not saturated, then it is invertible. However, this is not sufficient to conclude about the fans around the vertices of $X$. So we need more restrictions on the structures of the Kempe chains containing the vertices of $X$.

\begin{definition}
Let $X = (vv_0,\cdots,vv_{k-1})$ be a cycle with each $v_i$ missing color $i$. If there exists $i$ such that $v_{i+1} \not \in K_{v_i}(i,i+1)$, then $X$ is called \textit{reducible}. If we swap $K_{v_i}(i,i+1)$ we obtain a new coloring $\beta'$ which is called a reduction of $X$ where the sequence $X'=\{vv_0,\cdots,vv_i,vv_{i+1},\cdots,v_{k-1}$ is a fan inducing a cycle called the \textit{reduced cycle}.
\end{definition}

\begin{observation}
Let $X = (vv_0,\cdots,vv_{k-1})$ be a reducible cycle where each $v_i$ misses the color $i$, and $X'$ the reduced cycle. If $X'$ is invertible, then $X$ is invertible.
\end{observation}

\begin{proof}
As $X'$ is the reduced cycle of $X$, there exists $i$ such that the coloring $\beta'$ corresponding to the cycle $X'$ can be obtained from $\beta$ by swapping $C = K^\beta_{v_i}(i,i+1)$. We now consider the coloring $\beta''$, the invert of $X'$. In this coloring, $\beta''(vv_i) = i+1$, $\beta''(vv_{i+1}) = i$, and $m(v_{i+1}) = i+1$, so if we swap $K^{\beta''}_{v_i}(i,i+1) = C\cup \{vv_i,vv_{i+1}\}$, we obtain exactly $X^{-1}$.
\end{proof}

% \begin{definition}
% Let $X$ be a cycle in a coloring $\beta$ around a vertex $v$, and $Y$ a cycle around the same vertex in a coloring $\beta'$ equivalent to $\beta$ such that $|Y|<|X|$. If the fact that $Y$ is invertible in $\beta'$ implies the fact that $X$ is invertible in $\beta$, then $Y$ is called a \textit{predecessor} of $X$. If $X$ has no predecessor, then $X$ is called a \textit{tight} cycle.
% \end{definition}


\begin{definition}
Let $X$ be a cycle in a coloring $\beta$ around a vertex $v$, and $\{(\beta_1,Y_1),\cdots,(\beta_k,Y_k)\}$ a set of pair where each $Y_i$ is a cycle around $v$ in the coloring $\beta_i$. If the fact that for all $i$, $Y_i$ is invertible in $\beta_i$ implies that all the $\beta_i$ are equivalent to $\beta$, and $X$ is invertible in $\beta$, then $\{(\beta_1,Y_1),\cdots,(\beta_k,Y_k)\}$ is called a set of predecessor of $X$. If $X$ has no predecessor, then $X$ is called a \textit{tight} cycle.
\end{definition}

{\color{blue}(may need a stronger definition where a sequence of predecessor of $X$ is a sequence $(\beta_i,X_i)$ where the $X_i$ are disjoint cycles around $v$ strictly smaller than $X$ such that if each $X_i$ is invertible in $\beta_i$, then all the $\beta_i$ are equivalent to $\beta$, and $\Vv$ is invertible in $\beta$)}

So, to invert a cycle $X$, we can now only focus on the reduction of $X$ where the reduced cycle $X'$ is tight. In the coloring corresponding to $X'=\{vv_0,\cdots,vv_{k-1}\}$, each $v_{i+1}$ is in $K_{v_i}(i,i+1)$, and if we can invert $X'$, then we can invert $X$.

Note that if $X$ and $Y$ are two cycles around the same vertex $v$ in a coloring $\beta$, then as $X$ and $Y$ cannot have a common color, a reduction $\beta'$ of $Y$ is $X$-equivalent to $\beta$, so $X$ is invertible in $\beta$ if and only if it is invertible in $\beta'$.



\begin{observation}\label{obs:equiv_plus_reduction}
Let $X = (vv_0,\cdots,vv_{k-1})$ be a cycle around a vertex $v$ where each $v_i$ misses the color $i$, and let $\beta'$ be a coloring $\beta^{-1}(\{i,i+1\})\cup (X\setminus\{v_i\})$-equivalent to $\beta$ for some $i$. If $v_{i+1}\not \in K_{v_{i}}(i,i+1)$, then we swap $K_{v_{i}}(i,i+1)$ to obtain a coloring where $Y =  (vv_0,\cdots,vv_i,vv_{i+2},\cdots,vv_{k-1})$ is a predecessor of $X$.
\end{observation}



Again the proof of this observation is straightforward. Note that a tight cycle is never reducible. 

\begin{definition}
Let $X$ and $Y$ be two fans respectively around a vertex $y$ and $x$. $X$ and $Y$ are \emph{entangled} if for any pair of vertices $u\in X$ and $v\in Y$:\\
$m(x) = m(y)\implies x=y$.
\end{definition}


% Moreover, for any coloring $\beta$ and any cycle $X$ around a vertex $v$ in $\beta$, there exists a coloring $\beta'$ equivalent to $\beta$ which contains a cycle $Y$ such that:
% \begin{itemize}
%     \item $Y$ is tight,
%     \item $|Y|\leq|X|$ and
%     \item if $Y$ is invertible, then $X$ is invertible.
% \end{itemize}

==> main_thm.tex <==
\section{Main theorem}

In this section we prove Theorem~\ref{thm:Kempe}. Following \cite{bonamy2021vizing}, let $\gamma$ be a minimal coloring, and $v$ be a vertex adjacent to both a bad edge $vv'_1$ and an ugly edge $vv'_2$ where $m(v'_1) = \gamma(vv'_2)$. Let $\Vv' = (vv'_1,\cdots,vv'_{k'-1})$ be the fan around $v$ starting at $vv_1$. From \cite{bonamy2021vizing}, we have that $\Vv'$ is a saturated cycle. By Observation~\ref{obs:equiv_plus_reduction}, $\gamma$ is equivalent to a coloring $\beta$ where $\Vv = (vv_1,\cdots,vv_{k-1})$ is a tight predecessor of $\Vv'$ around $v$; without loss of generality, we can assume that each $v_i$ misses the color $i$. The principle of the proof is to show that $G = N[v] = K_{\Delta+1}$ using the two following Lemmas describing how cycles around $v$ interact with each other.

\begin{lemma}\label{lem:only_cycles}
For any $c\in [\Delta +1]\setminus\beta(\Vv)$, the cycle $\Vv$ is invertible or $X_v(c)$ is a cycle.
\end{lemma}


\begin{lemma}\label{lem:cycles_interaction}
Let $\Xx$ and $\Yy$ be two cycles around a vertex $v$, and let $z$ and $z'$ be two vertices of $\{\Vv,\Xx,\Yy\}$ .The fan $\Vv$ is invertible or for any $(z,z')$ in $\{\Vv^2,\Xx^2,\Xx\times\Vv,\Xx\times\Yy\}$, $X_z(m(z'))$ is a cycle containing $z'$.
\end{lemma}

We prove Lemma~\ref{lem:only_cycles} in section~\ref{sec:only_cycles_around_v} and Lemma~\ref{lem:cycles_interaction} in section~\ref{sec:cycles_interaction}

\begin{proof}
We have that if $\Vv'$ is invertible, then $\Vv'^{-1}(\gamma)$ is a coloring with strictly fewer bad edges than $\gamma$ which contradicts the minimality of $\gamma$. Moreover, by Observation~\ref{obs:equiv_plus_reduction}, the fan $\Vv'$ is not invertible only if the fan $\Vv$ is not invertible. Let us assume that $\Vv$ is not invertible, by Lemma~\ref{lem:only_cycles}, we have that all the fans around $v$ are cycle, moreover, if $\Xx$ and $\Yy$ are two cycles around $v$, and $x$ and $y$ are two vertices respectively of $\Xx$ and $\Yy$, by Lemma~\ref{lem:cycles_interaction}, the fan $X_x(m(y))$ is a cycle containing $y$. So for any pair of vertices $x,y$ of $N(v)$, $xy\in E(G)$ which directly implies that $G = N[v] = K_{\Delta+1}$. By construction, $G$ is $\Delta$-colorable, so $G$ is an even clique. However as all the fans around $v$ induce cycles, all the neighbors of $v$ are missing a different color. But this is impossible, as in a $(\Delta+1)$-coloring of an even clique, for any color $c$, the set of vertices missing the color $c$ is even. So $\Vv$ is invertible, and hence $\Vv'$ is invertible and $\gamma$ is not minimal; this concludes the proof.
\end{proof}









% \begin{lemma}\label{lem:cycles_around_v_starting_with_u}
% Let $\Uu = X_u(m(v)) = \{uu_1,\cdots,uu_{l-1}\}$ where $u = v_j$ is a vertex of $\Vv$, $w = u_s$ be a vertex of $\Uu$, then $\Vv$ is invertible or $Zz = X_v(m(w))$ is a cycle containing $w$.
% \end{lemma}


==> name.tex <==
en plus il faut savoir que tout cela n'est que foutaise :p

Je ne pense pas que ç

==> regularization.tex <==
\begin{figure}[h!]
\centering
%\begin{center}
 \hspace{-5mm}
 \uncover<1-2>
 {
 \begin{subfigure}[t]{0.15\textwidth}
\centering
\begin{tikzpicture}[node distance=6mm and 6mm, auto]
 \node[dot](s){};
 \node[dot,right=of s](b){}
 edge[pil] node {2} (s);
 \node[dot,above =of b](a){}
 edge[pil,above] node {1} (s);
 \node[dot,below =of b](c){}
 edge[pil] node {3} (s);
  \node[below= of c] (empty) {};
\end{tikzpicture}
%\caption{Graph $G$}
\end{subfigure}
%\hfill
 
 }


\uncover<2-2>
{
\begin{subfigure}[t]{0.2\textwidth}
\centering
%\hspace{5mm} 
\begin{tikzpicture}[node distance=6mm and 6mm, auto]
 \node[dot](s){};
 \node[dot,right=of s](b){}
 edge[pil] node {2} (s);
 \node[dot,above =of b](a){}
 edge[pil,above] node {1} (s);
 \node[dot,below =of b](c){}
 edge[pil] node {3} (s);
 
  \node[dot,right=of b](b2){}
  edge[pil] node {3} (b);
  \node[dot,right =of b2](s2){}
   edge[pil] node {2} (b2);
 \node[dot,above =of b2](a2){}
 edge[pil,above] node {1} (s2)
 edge[pil] node {2} (a);
 \node[dot,below =of b2](c2){}
 edge[pil,below] node {3} (s2)
 edge[pil,above] node {1} (c);
 \node[below= of c] (empty) {};
 
\end{tikzpicture}
%\caption{Step 1 : minimum degree increases to 2}
\end{subfigure}

}
\uncover<3->
{
%\hfill
\vspace*{-35ex}
%\hspace{9mm}
\begin{subfigure}[t]{0.5\textwidth}
\centering
\begin{tikzpicture}[node distance=5mm and 5mm, auto]
 \node[dot](s){};
 \node[dot,right=of s](b){}
 edge[pil] node {2} (s);
 \node[dot,above =of b](a){}
 edge[pil,above] node {1} (s);
 \node[dot,below =of b](c){}
 edge[pil] node {3} (s);
 
  \node[dot,right=of b](b2){}
  edge[pil] node {3} (b);
  \node[dot,right =of b2](s2){}
   edge[pil, below] node {2} (b2);
 \node[dot,above =of b2](a2){}
 edge[pil,above] node {1} (s2)
 edge[pil] node {2} (a);
 \node[dot,below =of b2](c2){}
 edge[pil,below] node {3} (s2)
 edge[pil,above] node {1} (c);
 
  \node[dot, right=of s2](s3){};
 \node[dot,right=of s3](b3){}
 edge[pil, below] node {2} (s3);
 \node[dot,above =of b3](a3){}
 edge[pil,above] node {1} (s3);
 \node[dot,below =of b3](c3){}
 edge[pil] node {3} (s3);
 
  \node[dot,right=of b3](b4){}
  edge[pil] node {3} (b3);
  \node[dot,right =of b4](s4){}
   edge[pil] node {2} (b4);
 \node[dot,above =of b4](a4){}
 edge[pil,above] node {1} (s4)
 edge[pil] node {2} (a3);
 \node[dot,below =of b4](c4){}
 edge[pil,below] node {3} (s4)
 edge[pil,above] node {1} (c3);
  \node[below= of c] (empty) {};
 \path (a) edge[pil, bend left=30] node {3}  (a3) ;
 \path (a2) edge[pil, bend left=30] node {3}  (a4) ;
 \path (b) edge[pil, bend left=30] node {1}  (b3) ;
 \path (b2) edge[pil, bend left=30] node {1}  (b4) ;
 \path (c) edge[pil, bend right=30, below] node {2}  (c3) ;
 \path (c2) edge[pil, bend right=30,below] node {2}  (c4) ;
\end{tikzpicture}
%\caption{Step 2 (final): a 3-regular graph}
\end{subfigure}

}

%\caption{Construction of a $3$-regular $3$-edge colourable graph from a $3$-edge colourable graph}
\label{fig:regular}
%\end{center}

\end{figure}


